EuroFlood: A queryable index for satellite-derived flood depths in Europe

Satellite-derived observations of flood water depth support flood model validation and impact assessment, yet the only open continental-scale archive of such observations, the flood-depth maps of the Copernicus Emergency Management Service, is distributed as several thousand raster files whose sole spatial metadata is a coordinate encoded in each filename. This paper presents EuroFlood, an open-source Python library and a published spatial index that make the archive queryable. The index records which archived events inundated each grid cell, enabling event discovery, footprint reconstruction, and recurrence analysis directly from the index, while high-resolution depth rasters are retrieved only when needed. It reproduces the archived event footprints losslessly at its grid. A region-level corroboration audit against an independent flood-impact database shows stronger agreement for river floods, while results for flash floods are less conclusive. Applications demonstrate continental recurrence mapping, comparison of observed with modelled flood extents, and event-based exposure assessment.

==> benchmark-rows.tex <==
city (Zutphen) & 30 & 19.3 & 0.13 & 13 & 7 & 10 & 67 & 9 \\
metro (Cologne) & 12 & 19.3 & 0.13 & 8 & 0 & 25 & 0 & 12 \\
country (NL) & 126 & 20.8 & 1.51 & 275 & 27 & 46 & 100 & 84 \\
\bottomrule

